Dynamic Prediction of ICU Mortality Risk Using Domain Adaptation

Early recognition of risky trajectories during an Intensive Care Unit (ICU) stay is one of the key steps towards improving patient survival. Learning trajectories from physiological signals continuously measured during an ICU stay requires learning time-series features that are robust and discriminative across diverse patient populations. Patients within different ICU populations (referred here as domains) vary by age, conditions and interventions. Thus, mortality prediction models using patient data from a particular ICU population may perform suboptimally in other populations because the features used to train such models have different distributions across the groups. In this paper, we explore domain adaptation strategies in order to learn mortality prediction models that extract and transfer complex temporal features from multivariate time-series ICU data. Features are extracted in a way that the state of the patient in a certain time depends on the previous state. This enables dynamic predictions and creates a mortality risk space that describes the risk of a patient at a particular time. Experiments based on cross-ICU populations reveals that our model outperforms all considered baselines. Gains in terms of AUC range from 4% to 8% for early predictions when compared with a recent state-of-the-art representative for ICU mortality prediction. In particular, models for the Cardiac ICU population achieve AUC numbers as high as 0.88, showing excellent clinical utility for early mortality prediction. Finally, we present an explanation of factors contributing to the possible ICU outcomes, so that our models can be used to complement clinical reasoning.

==> table1.tex <==
\begin{table*} [ht!]
\caption{Average patient physiological data. Mean, first and third quartiles within each physiological parameter. Mortality rate (MR) is concentrated in the Medical ICU (49.6\% of the deaths).}
\centering
\begin{tabular}{lllll} \hline
&Cardiac&Coronary&Medical&Surgical\\\hline\\
N     & 577 (MR=14.6\%)& 874 (MR=7.8\%)& 1,481 (MR=49.6\%)& 1,067 (MR=28.0\%)\\
Age   &69.22 (59$-$81)& 67.91 (56$-$79)& 62.83 (51$-$78)& 60.50 (48$-$76)\\

Male  & 333 (57.7\%)& 530 (60.6\%)& 753 (50.8\%)& 630 (59.0\%)\\
\hline\\
\multicolumn{5}{l}{\bf{Physiological data}}\\
Albumin (g/dL) & 3.31 (2.9$-$3.6) & 2.92 (2.4$-$3.5) & 2.92 (2.5$-$3.3) & 2.99 (2.5$-$3.5) \\
Alkaline phosphatase (IU/L) & 92.44 (59$-$102) & 74.93 (46$-$83) & 126.15 (64$-$138) & 91.43 (52$-$96) \\
Alanine transaminase (IU/L) & 128.28 (19$-$78) & 89.16 (18$-$45) & 164.87 (16$-$61) & 191.52 (17$-$84) \\
%Aspartate transaminase (IU/L) & 247.46 (26$-$165) & 161.94 (28$-$86) & 222.62 (24$-$87) & 252.87 (24$-$117) \\
Bilirubin (mg/dL) & 0.87 (0.4$-$0.9) & 1.01 (0.4$-$1.1) & 2.44 (0.4$-$1.6) & 1.85 (0.5$-$1.5) \\
Blood urea nitrogen (mg/dL) & 29.92 (16$-$36) & 18.76 (12$-$21) & 32.59 (14$-$42) & 20.36 (11$-$24) \\
Cholesterol (mg/dL) & 163.59 (134$-$189) & 150.14 (114$-$174) & 141.04 (111$-$169) & 157.87 (122$-$184) \\
Creatinine (mg/dL) & 1.58 (0.8$-$1.6) & 1.04 (0.7$-$1.1) & 1.64 (0.7$-$1.7) & 1.12 (0.7$-$1.1) \\
Invasive diast. press. (mmHg) & 62.65 (53$-$74) & 58.85 (51$-$66) & 54.97 (48$-$70) & 59.65 (52$-$72) \\
Fractional inspired O2 & 0.82 (0.5$-$1.0) & 0.91 (1.0$-$1.0) & 0.72 (0.5$-$1.0) & 0.72 (0.5$-$1.0) \\
Serum glucose (mg/dL) & 165.74 (114$-$191) & 129.28 (103$-$145) & 155.02 (104$-$175) & 148.85 (114$-$167) \\
Serum bicarbonate (mmol/L) & 23.31 (21$-$26) & 23.41 (22$-$25) & 22.74 (19$-$26) & 23.44 (21$-$26) \\
Hematocrit (\%) & 34.48 (30.7$-$37.8) & 29.32 (25.3$-$32.8) & 31.82 (27.9$-$36) & 33.01 (29.1$-$36.8) \\
Heart rate (bpm) & 84.32 (69$-$97) & 85.43 (79$-$91) & 95.61 (80$-$110) & 87.83 (74$-$100) \\
Serum potassium (mEq/L) & 4.28 (3.8$-$4.5) & 4.49 (4$-$4.7) & 4.19 (3.6$-$4.5) & 4.07 (3.6$-$4.3) \\
Lactate (mmol/L) & 2.76 (1.4$-$3) & 2.76 (1.5$-$3.3) & 2.58 (1.3$-$2.8) & 2.65 (1.3$-$3.1) \\
Serum magnesium (mmol/L) & 1.90 (1.7$-$2.1) & 2.22 (1.8$-$2.4) & 1.95 (1.6$-$2.1) & 1.80 (1.5$-$2) \\
Invasive mean press. (mmHg) & 86.14 (73$-$99) & 78.86 (69$-$86) & 86.58 (68$-$96) & 87.13 (73$-$98) \\
Serum sodium (mEq/L) & 137.82 (135$-$140) & 138.42 (136$-$140) & 138.96 (136$-$142) & 139.33 (137$-$142) \\
Non-invasive diast. press. (mmHg) & 61.15 (49$-$72) & 52.21 (44$-$59) & 62.03 (50$-$72) & 62.42 (52$-$73) \\
Non-invasive mean press. (mmHg) & 78.93 (67$-$89) & 71.53 (62$-$79) & 80.55 (68$-$91) & 82.78 (71$-$94) \\
Non-invasive syst. press. (mmHg) & 117.46 (101$-$134) & 110.88 (96$-$125) & 121.78 (104$-$138) & 126.72 (108$-$145) \\
Partial press. of art. CO2 (mmHg) & 40.61 (35$-$45) & 41.20 (36$-$45) & 42.50 (34$-$48) & 41.01 (35$-$45) \\
Partial press. of art. O2 (mmHg) & 181.58 (89$-$248) & 295.46 (218$-$387) & 147.68 (78$-$185) & 188.24 (101$-$250) \\
Arterial pH (0-14)& 7.84 (7.31$-$7.43) & 7.39 (7.35$-$7.44) & 7.44 (7.3$-$7.42) & 7.46 (7.32$-$7.43) \\
Platelets (cells/nL) & 241.44 (181$-$283) & 170.36 (117$-$208) & 230.89 (143$-$287) & 219.19 (150$-$268) \\
Respiration rate (bpm) & 19.74 (16$-$23) & 17.55 (14$-$20) & 21.10 (17$-$24) & 18.95 (16$-$21) \\
O2 saturation in hemoglobin (\%) & 96.25 (96$-$98) & 97.48 (97$-$98) & 94.84 (94$-$98) & 96.99 (97$-$98) \\
Invasive systolic press. (mmHg) & 117.65 (100$-$139) & 117.16 (105$-$127) & 107.45 (95$-$137) & 123.33 (108$-$148) \\
Temperature ($^o$C) & 36.38 (36$-$37.1) & 35.57 (35.5$-$36.6) & 36.77 (36.2$-$37.4) & 36.51 (36.1$-$37.4) \\
Troponin-I ($\mu$g/L) & 10.05 (0.8$-$12.4) & 6.77 (0.8$-$10.1) & 5.59 (0.8$-$7) & 7.02 (0.4$-$6.7) \\
Troponin-T ($\mu$g/L) & 2.78 (0.17$-$2.8) & 1.51 (0.04$-$0.59) & 0.33 (0.04$-$0.25) & 0.22 (0.03$-$0.14) \\
Urine output (mL) & 365.62 (100$-$500) & 497.92 (120$-$615) & 255.39 (70$-$325) & 389.29 (100$-$500) \\
White blood cell (cells/nL) & 12.31 (8.5$-$14.3) & 12.98 (9.2$-$15.5) & 13.33 (7.8$-$17) & 12.37 (8.4$-$15.1)\\
\hline
\end{tabular}
\label{tab:physionet}
\end{table*}

